Simplicity of random hypergraphs

Random hypergraphs extend the classical notion of random graphs by allowing hyperedges to join more than two vertices, making them well-suited for modeling higher-order interactions in complex systems. Despite their broad applicability, many structural properties of random hypergraphs remain less understood than in the graph setting. One such property is simplicity: the absence of self-loops, multi-hyperedges, and, in the hypergraph context, degenerate hyperedges where hyperedges contain a copy of the same vertex at least twice. While the behaviour of the number of such self-loops and multi-hyperedges is well understood for random graphs through the configuration model, analogous results for hypergraphs are comparatively sparse. In this work, we study both undirected and directed hypergraphs generated by the configuration model with prescribed vertex and hyperedge degrees. We derive exact, explicit expressions for the expected number of self-loops, multi-hyperedges and degenerate hyperedges, extending classical results from the graph setting. In addition, an asymptotical analysis shows that, under mild moment conditions on the degree distribution, the expected fraction of self-loops, multi-hyperedges and degenerate hyperedges vanishes as the number of vertices grows. Our results provide a systematic understanding of simplicity in directed and undirected hypergraph models.

==> undirected/statistics.tex <==
\label{section:undirected_stats}
In this section, we consider a uniformly random undirected hypergraph $H=(V,E)$ with $n=|V|$ vertices and some degree sequence $\vb*{d}$. We study the expected number of degenerate hyperedges and multi-hyperedge pairs in this hypergraph. We present exact results, as well as asymptotic results for regular hypergraphs in which all hyperedges have the same degrees.

A hyperedge is \textit{degenerate} if it contains some vertex at least twice~\cite{chodrow2020configuration}. Degenerate hyperedges could be interpreted as `self-loops' in undirected hypergraphs.
\\
\begin{definition}[Degenerate hyperedge]
    A hyperedge $e \in E$ is called \textit{degenerate} if $\exists v \in V: m_{v}(e) \geq 2$.
\end{definition}
The total number of degenerate hyperedges is denoted by
\begin{align*}
    DH_n = \sum_{e \in E} \mathds{1}_{\{\exists v \in V: \, m_v(e) \geq 2\}}.
\end{align*}

Two hyperedges are a \textit{multi-hyperedge pair} if they are equal as multisets. 
\\
\begin{definition}[Multi-hyperedge pair]
    Two hyperedges $e_1,e_2 \in E$ are a multi-hyperedge pair if $e_1=e_2$.
\end{definition}
The total number of multi-hyperedge pairs is denoted by 
\begin{align*}
    M_n = \frac{1}{2} \sum_{e \in E} \sum_{e' \in E \backslash \{e\}} \mathds{1}_{\{e=e'\}}.
\end{align*}
Note that if $k$ hyperedges are equal then this results in $(k-1)!$ multi-hyperedge pairs.
